Stochastic Optimization for Performative Prediction

In performative prediction, the choice of a model influences the distribution of future data, typically through actions taken based on the model's predictions. We initiate the study of stochastic optimization for performative prediction. What sets this setting apart from traditional stochastic optimization is the difference between merely updating model parameters and deploying the new model. The latter triggers a shift in the distribution that affects future data, while the former keeps the distribution as is. Assuming smoothness and strong convexity, we prove rates of convergence for both greedily deploying models after each stochastic update (greedy deploy) as well as for taking several updates before redeploying (lazy deploy). In both cases, our bounds smoothly recover the optimal $O(1/k)$ rate as the strength of performativity decreases. Furthermore, they illustrate how depending on the strength of performative effects, there exists a regime where either approach outperforms the other. We experimentally explore the trade-off on both synthetic data and a strategic classification simulator.

==> discussion.tex <==
% !TEX root = main.tex
\newpage
\section{Discussion and future work}

In this work we have proposed the first study of stochastic optimization for performative prediction, a non-stationary setting where updates to model parameters might  trigger a distribution shift. We have analyzed different variants of SGD under this setting and identified the number of update steps taken between deployments as an important algorithmic design choice. 
However, there are many more open questions and interesting aspects to study in this new framework. 

Building on the insights from this work one might aim to find the best deployment strategies for SGD to improve the sample efficiency of the method. In this context adaptive deployment schedules would be an interesting direction. \textit{Could one anticipate performative effects by taking greedy decisions based on planned model updates?} These updates give valuable  information on the expected distribution shift which in turn could be used to pick an appropriate stepsize or decide the number of steps to take before the next deployment. 

An orthogonal dimension of the problem would be to incorporate time dependent drift into the analysis. This would mean to take into account that performative effects are not instantaneous, but pronounced over time. As a consequence, samples collected in lazy SGD after deploying classifier $\theta_k$  are not sampled i.i.d from $\D(\theta_k)$, but, instead, sampled from a drifting distribution that continuously approaches $\cD(\theta_k)$, such as illustrated in Figure \ref{fig:generalshift}. This model comes with interesting technical challenges and design choices for modelling time dependent drift.
 
Again another direction would involve social aspect of stochastic optimization in performative prediction. \textit{Do we want to incentivize people to adapt to noisy models? what are the consequences and how can we design algorithms to avoid undesirable effects?}











%%%%%%%%%%%%%%%%%%%
\begin{figure}[t!]
\centering
\begin{tikzpicture}[
declare function={
normal(\x,\m,\s,\c) = \c*1/(2*\s*sqrt(pi))*exp(-(\x-\m)^2/(2*\s^2));
}]
\begin{axis}[
  no markers, 
domain=-1:11, 
samples=100,
  axis lines=left, 
xlabel=\empty, 
ylabel=\empty,
  every axis y label/.style={at=(current axis.above origin),anchor=south},
  every axis x label/.style={at=(current axis.right of origin),anchor=west},
  xtick={2,8}, 
xticklabels={},
ytick=\empty,
  enlargelimits=false, clip=false, axis on top,
  grid = none,
width=0.6\textwidth,
height=0.2\textwidth,
hide y axis
 ]
\addplot [c1, thick, dotted] (x,{normal(x, 2, 0.7,1)});
\addplot [c1, thick, dotted] (x,{normal(x, 8, 0.7,1)});
\addplot [c2, fill=c2, fill opacity=0.5] (x,{normal(x, 3.5, 0.7,1)});
\node [above, text = c1] at (2,{normal(2, 2, 0.7,1)}) {$\cD_{k-1}$};
\node [above, text = c1] at (3.5,{normal(3.5, 3.5, 0.7,1)}) {$\cD_{k}$};
\node [above, text = c1] at (8,{normal(8, 8, 0.7,1)}) {$\cD(\theta_k)$};
\draw[color=c1, ->] (5,0.15) -- (6.5,0.15);
\node [above, text = c1] at (5.75,0.15) {$\alpha$};
\end{axis}
\end{tikzpicture}
\caption{Time-dependent Drift Model for adapting to a new classifier $\theta_{k} := G(\cD_{k-1})$ with $\alpha\in(0,1]$ increasing over time. }
\label{fig:generalshift}
\end{figure}
%%%%%%%%%%%%%%%%%%%

